Modeling Multiple Views via Implicitly Preserving Global Consistency and Local Complementarity

While self-supervised learning techniques are often used to mining implicit knowledge from unlabeled data via modeling multiple views, it is unclear how to perform effective representation learning in a complex and inconsistent context. To this end, we propose a methodology, specifically consistency and complementarity network (CoCoNet), which avails of strict global inter-view consistency and local cross-view complementarity preserving regularization to comprehensively learn representations from multiple views. On the global stage, we reckon that the crucial knowledge is implicitly shared among views, and enhancing the encoder to capture such knowledge from data can improve the discriminability of the learned representations. Hence, preserving the global consistency of multiple views ensures the acquisition of common knowledge. CoCoNet aligns the probabilistic distribution of views by utilizing an efficient discrepancy metric measurement based on the generalized sliced Wasserstein distance. Lastly on the local stage, we propose a heuristic complementarity-factor, which joints cross-view discriminative knowledge, and it guides the encoders to learn not only view-wise discriminability but also cross-view complementary information. Theoretically, we provide the information-theoretical-based analyses of our proposed CoCoNet. Empirically, to investigate the improvement gains of our approach, we conduct adequate experimental validations, which demonstrate that CoCoNet outperforms the state-of-the-art self-supervised methods by a significant margin proves that such implicit consistency and complementarity preserving regularization can enhance the discriminability of latent representations.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> method_old.tex <==
\section{Method}
In this paper, we focus on learning feature representations that can model view-invariant factors. As shown in Figure \ref{fig:algoframe}, we learn representations by two aspects, i.e., local consistency and global alignment, and we show an example of learning from three views: Red-Green-Blue (RGB) view of the input image, the luminance channel (L) view of an image and the ab-color channel (ab) view. A detailed algorithm of LGCAN is given as Algorithm \ref{alg:lcgan} in Appendix \ref{appendix:nf}, Formally, we consider the multi-view dataset ${X^m} = \left[ {x_1^m,x_2^m,...,x_N^m} \right]$, where $X^m$ represents the sample collection from the $m$-th view, and ${x_i^m}$, $i=1,...,n$ represents the $i$-th sample of the $m$-th view. $N$ is the number of samples in the $m$-th view. Also, we denote $X^m$ as a random variable sampled \textit{i.i.d} from the distribution $\mathcal{P}\left(X^m \right) $. Also, we suppose ${x_i} = \left[ {x_i^1;x_i^2;x_i^3} \right]$ and $X = \left[ {{x_1},{x_2},...,{x_N}} \right]$, and we denote $X$ as a variable that is sampled \textit{i.i.d} from distribution $\mathcal{P}\left(X \right) $.

\subsection{Global consistency preserving network}
The idea behind global alignment is to learn a feature representation that captures information shared between multi-view samples globally. We aim to align $\mathcal{P}\left(X^1 \right) $, $\mathcal{P}\left(X^2 \right) $ and $\mathcal{P}\left(X^3 \right) $ in the latent space. Based on the Wasserstein distance, we call the method of global alignment as $WD-Alignment$. Figure \ref{fig:algow} depicts the framework of $WD-Alignment$. The theoretical analysis for adopting Wasserstein distance as our discrepancy metric is provided in Appendix \ref{appendix:ta}.

For $\mathcal{P}\left(X^i \right) $, we denote ${{H^i} = {f_\vartheta }\left( {{f_\omega }\left( {{X^i}} \right)} \right)}$ and $\mathcal{P}\left(H^i\right) $ as the distribution in latent space that are induced by ${{f_\vartheta }}$ and ${{f_\omega }}$, where $i \in \left\{ {1,2,3} \right\}$, the $p{\rm{th}}$ Wasserstein distance can be defined as:
\begin{equation}
\begin{aligned}
{W_p}\left( H^1,H^2 \right)
= {\left( {\mathop {\inf }\limits_{\mu \left( {h^i,h^j} \right) \in \Pi \left( {h^i,h^j} \right)} \int {c{{\left( {h^i,h^j} \right)}^p}d\mu } } \right)^{\frac{1}{p}}}
\end{aligned}
\end{equation}
where $c\left( {h^i,h^j} \right)$ represents the distance of two patterns and $\Pi \left( {h^i,h^j} \right)$ denotes the set of all joint distributions $\mu \left( {h^i,h^j} \right)$ that satisfy $\mathcal{P}\left(H^i \right) = \int_h^j {\mu \left( {h^i,h^j} \right)dh^j}, {\mathcal{P}\left(H^j \right)} = \int_h^i {\mu \left( {h^i,h^j} \right)dh^i}$.

Based on the Kantorovich-Rubinstein theorem, the dual form of Wasserstein distance can be written as:
\begin{equation}
\begin{array}{l}
{W_p}\left( {\mathcal{P}\left( {{H^i}} \right),\mathcal{P}\left( {{H^j}} \right)} \right)\\
= \mathop {\sup }\limits_{\left\| \xi_{ij} \right\|{}_L \le 1} \mathop \mathbb{E} \limits_{{h^i} \sim \mathcal{P}\left( {{h^i}} \right)} \left[ {\xi_{ij} \left( {{h^i}} \right)} \right] - \mathop \mathbb{E} \limits_{{h^j} \sim \mathcal{P}\left( {{H^j}} \right)} \left[ {\xi_{ij} \left( {{H^j}} \right)} \right]
\end{array}
\end{equation}
where $\xi_{ij} :{h} \to R$ is the 1-Lipschitz function and satisfies ${\left\| \xi_{ij} \right\|_L} = \mathop {\sup }\limits_{h_i \ne h_j} {{\left| {\xi_{ij} \left( h_i \right) - \xi_{ij} \left( h_j \right)} \right|} \mathord{\left/
		{\vphantom {{\left| {\xi_{ij} \left( h_i \right) - \xi_{ij} \left( h_j \right)} \right|} {\left| {h_i - h_j} \right|}}} \right.
		\kern-\nulldelimiterspace} {\left| {h_i - h_j} \right|}} \le 1$.
Then, the objective function of the global alignment module is defined as:
\begin{equation}
\mathop {\min }\limits_{\xi_{12},\xi_{13},\xi_{23}} {L_{ga}}= \sum\limits_{i=1,i < j}^3 {W_p}\left( {\mathcal{P}\left( {{H^i}} \right),\mathcal{P}\left( {{H^j}} \right)} \right) 
\end{equation}

\subsection{Local consistency preserving network}
The idea behind local consistency is to learn a feature representation that captures information shared between multi-view samples in an instance-based manner. To this end, we focus on maximizing mutual information (MI) between the local features and the global features of each multi-view sample from two aspects. We begin by reviewing the unsupervised feature representations paradigm, focusing on estimating and maximizing mutual information. Then, we introduce the proposed local consistency module, which consists of two parts, including $Full-View$ consistency module and $Intra-View$ consistency module.

%\begin{figure}
%	\begin{center}
%		\centerline{\includegraphics[width=0.97\columnwidth]{algoi}}
%		\vskip -0.15in
%		\caption{Learning representations based on \textbf{Intra-View} MI estimation and maximization.}
%		\label{fig:algoi}
%	\end{center}
%	\vskip 0.1in
%\end{figure}
% \vspace{-1cm}

Specifically, given a dataset with three-views $\left\{ {{X^1},{X^2},{X^3}} \right\}$, we first encode every input into the latent space to obtain the embedding with $d \times c \times c$ dimensions by a feature extraction network ${f_\omega }$, where $d$ represents the number of channels, $c \times c$ represents the size of the feature map. Thus for each input, we obtain $c^2$ local $d$-dimensional vectors. Then, we map the obtained embedding into a $d$-dimensional global feature vector by a mapping network ${f_\vartheta}$. The local vector is regarded as a random variable $h$ sampled \textit{i.i.d} from the distribution $\mathcal{P}\left(h \right) $. The global vector is regarded as a random variable $g$ sampled \textit{i.i.d} from the distribution $\mathcal{P}\left(g \right) $. We maximize the mutual information between the random variable $h$ and the random variable $g$. We employ the Jensen-Shannon divergence (JSD) as the MI estimator since it is more stable, \cite{ib18, rdh19}. Although other MI estimation methods have good but inconsistent performance, the stability of JSD makes it more interpretable and reliable. Inspired from \cite{sn16}, we define a JSD MI estimator as:
\begin{equation}
	\begin{array}{l}
		I\left( {h;g} \right): = I_{\omega, \vartheta, w}^{JSD} = {\mathbb{E}_\mathcal{P}}\left[ { - sp\left( { - {T_w}\left( {{f_\omega }\left( x \right),{f_\vartheta }\left( {{f_\omega }\left( x \right)} \right)} \right)} \right)} \right]\\
		- {\mathbb{E}_{\mathcal{P} \times \mathcal{P}}}\left[ {sp\left( { - {T_w}\left( {{f_\omega }\left( {x'} \right),{f_\vartheta }\left( {{f_\omega }\left( x \right)} \right)} \right)} \right)} \right]
	\end{array}
\end{equation}
where $x$ and ${x'}$ are the input samples, $\mathcal{P}$ represents the distribution of the input samples, ${\mathcal{P} \times \mathcal{P}}$ represents the joint distribution, $sp\left( z \right) = log\left(1+e^z \right) $ is the softplus function, and ${{T_w}}$ is a discrimination network.

%For the $Intra-View$ consistency module, as shown in Figure \ref{fig:algoi}, we estimate and maximize the mutual information for each view separately. Suppose the $x_i^m$ is the $i$-th sample from the $m$-th view, then we first encode it into the latent space and obtain the $d \times c \times c$-dimensional embedding and the $d$-dimensional global feature vector. We first compute the global mutual information. Specifically, the embedding is flattened, and concatenated with the global feature vector, i.e., $F_{co}\left[ {F_{fl}\left({f_\omega }\left( x_i^m \right)\right),{f_\vartheta }\left( {{f_\omega }\left( x_i^m \right)} \right)}\right] $, where $F_{co}$ represents the concatenating operation and $F_{fl}$ represents the flattening operation. We regard this pair as positive pair, and the negative pairs are generated by combining ${{f_\vartheta }\left( {{f_\omega }\left( x_i^m \right)} \right)}$ with the embedding ${{f_\omega }\left( {{x_j^m}} \right)}$, where $x_j^m$ is a different image of the same view. Then, a discrimination network ${{T_w^G}}$ is used to score the pairs. We solve the following objective function:
%\begin{equation}
%	\begin{array}{l}
%		\mathop {\max }\limits_{{f_\omega }, {f_\vartheta }, T_w^G} {I_{global}^{JSD}} \\=\sum\limits_{m = 1}^3 {\left\{ {\mathop \mathbb{E}\limits_{x_i^m \sim \mathcal{P}\left( {{X^m}} \right)} {\left\{ { - sp\left( { - {T_w^G}\left( {\rm A}\left( {x_i^m,x_i^m} \right) \right)} \right)} \right.} } \right.} \\
%		- \left. {\left. {\mathop \mathbb{E}\limits_{x_j^m \sim \mathcal{P}\left( {{X^m}} \right),x_j^m \ne x_i^m} {sp\left( { - {T_w^G}\left( {\rm A}\left( {x_i^m,x_j^m} \right) \right)} \right)} } \right\} } \right\}
%	\end{array}
%\end{equation}
%where ${\rm A}\left( {x_i^m,x_j^m} \right) = F_{co}\left[ {F_{fl}\left({f_\omega }\left( x_i^m \right)\right),{f_\vartheta }\left( {{f_\omega }\left( x_j^m \right)} \right)}\right]$, $N$ is the number of positive samples, and $m$ is the number of views. Then we compute the local mutual information. We regard the obtained $d \times c \times c$-dimensional embedding as $c^2$ local $d$-dimensional vectors, and then we concatenate the $d$-dimensional global feature vector with each local $d$-dimensional vectors separately to obtain the positive pairs. The negative pairs are generated by combining the global feature vector with the local vectors from different images of the same view. Then, a discrimination network ${{T_w^L}}$ is used as a discriminator to score the pairs. The optimization is as follows:
%\begin{equation}
%	\begin{array}{l}
%		\mathop {\max }\limits_{{f_\omega },{f_\vartheta },T_w^L} {I_{local}^{JSD}}= \\
%		\sum\limits_{m = 1}^3 {\left\{ {\mathop \mathbb{E} \limits_{x_{{i}}^m \sim P\left( {{X^m}} \right)} \sum\limits_{{a},{b} = 1,}^c {\left\{ { - sp\left( { - {T_w^L}\left( {{\rm B}^{a,b}}\left( {x_i^m,x_j^m} \right) \right)} \right)} \right.} } \right.} \\
%		- \mathop \mathbb{E} \limits_{x_j^m \ne x_{{i}}^m,\hfill\atop
%			x_j^m \sim P\left( {{X^m}} \right)\hfill} \left. {\left. {\sum\limits_{{a},{b} = 1}^c {sp\left( { - {T_w^L}\left({{\rm B}^{a,b}}\left( {x_j^m,x_i^m} \right) \right)} \right)} } \right\}} \right\}
%	\end{array}
%\end{equation}
%where ${{\rm B}^{a,b}}\left( {x_i^m,x_j^m} \right) = {F_{co}}\left[ {f_w^{^{a,b}}\left( {x_i^m} \right),{f_\vartheta }\left( {{f_\omega }\left( {x_j^m} \right)} \right)} \right]$, ${{f_\omega }^{{a},{b}}\left( {x_{{i}}^m} \right)}$ represent the local vectors at positions $\left( i_1,i_2\right) $ of the embedding ${f_\omega }\left( {x_{{i_1}}^m} \right)$. Also, we impose statistical constraints onto the learned embedding by implicitly training the encoder so that the push-forward distribution ${{\mathcal{U}_{\vartheta,\omega,\mathcal{P}}}}$ matches a prior $\mathcal{V}$. To do this, we first sample several samples from the prior $\mathcal{V}$. Then, based on the discrimination network ${D_\phi }$, we optimize the follows.
%\begin{equation}
%	\begin{array}{l}
%		\mathop {\min }\limits_{{f_\omega },{f_\vartheta }}\mathop {\max }\limits_{D_\phi} D\left( {\mathcal{V}\left| {{\mathcal{U}_{\vartheta,\omega,\mathcal{P}}}} \right.} \right) =\\
%		\mathop \mathbb{E} \limits_{{x_v} \sim \mathcal{V}} \left( {\log {D_\phi }\left( {{x_v}} \right)} \right) + \mathop \mathbb{E} \limits_{{x^m} \sim \mathcal{P}\left( {{X^m}} \right)} \left( {\log \left( {1 - {D_\phi }\left( {{f_\vartheta }\left( {{f_\omega }\left( {{x^m}} \right)} \right)} \right)} \right)} \right)
%	\end{array}.
%\end{equation}
%
%And the objective function of $Intra-View$ is defined as
%\begin{equation}
%	\mathop {\max }\limits_{{f_\omega },{f_\vartheta },{D_\phi}, T_w^G,T_w^L }{L_{iv}} = I_{global}^{JSD} + I_{local}^{JSD} - D\left( {\mathcal{V}\left| {{\mathcal{U}_{\vartheta,\omega,\mathcal{P}}}} \right.} \right).
%\end{equation}

\begin{figure}[htb]
	\vskip -1in
	\begin{center}
		\centerline{\includegraphics[width=0.97\columnwidth]{algof}}
		\caption{Learning representations based on \textbf{Full-View} MI estimation and maximization.}
		\label{fig:algof}
	\end{center}
	\vskip -0in
\end{figure}

For the $Full-View$ consistency module, as shown in Figure \ref{fig:algof}, we first encode the three-views samples into the latent space and obtain three $d \times c \times c$-dimensional embedding and three $d$-dimensional global feature vectors, respectively. Then we concatenate the three global vectors to obtain the $3d$-dimensional $Full-View$ global vector. For the computation of the global mutual information, the flattened three embeddings are concatenated with the $Full-View$ global feature vector to obtain the three positive pairs. Combining the $Full-View$ global feature vector with embedding from other samples of three views generates the negative pairs. Then, a discrimination network ${{V_w^G}}$ scores the pairs. We denote this as:
\begin{equation}
	\begin{array}{l}
		A\left( {x_i^m,x_i^1,x_i^2,x_i^3} \right) = \\
		{F_{co}}\left[ {{F_{cl}}\left( {x_i^m} \right),{f_\vartheta }\left( {{f_\omega }\left( {x_i^1} \right)} \right),{f_\vartheta }\left( {{f_\omega }\left( {x_i^2} \right)} \right),{f_\vartheta }\left( {{f_\omega }\left( {x_i^3} \right)} \right)} \right]
	\end{array}
\end{equation}
Then, we optimize the follows.
\begin{equation}
	\begin{array}{l}
		\mathop {\max }\limits_{{f_\omega },{f_\vartheta },V_w^G} \bar I_{global}^{JSD}= \mathop \mathbb{E} \limits_{x_i^{m} \sim \mathcal{P}\left( X^m \right)\hfill\atop
			m \in \left\{ {1,2,3} \right\}\hfill} \left\{ { - sp\left( { - {V_w^G}\left( A\left( {x_i^m,x_i^1,x_i^2,x_i^3} \right) \right)} \right)} \right.\\
		- \mathop \mathbb{E} \limits_{ j \ne i \hfill\atop
			{x_j^{m} \sim \mathcal{P}\left( {{X^{m}}} \right)\hfill\atop
				m \in \left\{ {1,2,3} \right\}\hfill}} \left. {sp\left( { - {V_w^G}\left( A\left( {x_j^m,x_i^1,x_i^2,x_i^3} \right) \right)} \right)} \right\}
	\end{array}
\end{equation}

To compute the local mutual information of $Full-View$, we regard the obtained three $3c$-dimensional embedding as $3 \times c^2$ local $d$-dimensional vectors. Then we concatenate the global feature vector with each local $d$-dimensional vector separately to obtain the positive pairs. Combining the global feature vector with the local vectors from other samples of three views generates the negative pairs. Then, a discrimination network ${{V_w^L}}$ score the pairs. Optimization is applied as follows:
\begin{equation}
	\begin{array}{l}
		\mathop {\max }\limits_{{f_\omega },{f_\vartheta },V_w^L} \bar I_{local}^{JSD} = \begin{array}{l}
			\mathop \mathbb{E} \limits_{x_i^m \sim P\left( {{X^m}} \right)\hfill\atop
				m \in \left\{ {1,2,3} \right\}\hfill} \left\{ { - sp\left( { - V_w^L\left( {{{\rm B}^{a,b}}\left( {x_i^m,x_i^1,x_i^2,x_i^3} \right)} \right)} \right)} \right. - \\
			\left. {\mathop \mathbb{E} \limits_{x_i^m \sim P\left( {{X^m}} \right)\hfill\atop
					{m \in \left\{ {1,2,3} \right\}\hfill\atop
						i \ne j\hfill}} - sp\left( { - V_w^L\left( {{{\rm B}^{a,b}}\left( {x_j^m,x_i^1,x_i^2,x_i^3} \right)} \right)} \right)} \right\}
		\end{array}
	\end{array}
\end{equation}

\begin{figure}[htb]
	\vskip-1in
	\begin{center}
		\centerline{\includegraphics[width=0.97\columnwidth]{algow}}
		\vskip 0.04in
		\caption{The WD-Alignment module globally aligns the distributions in the latent space by calculating the Wasserstein distances between different views.}
		\label{fig:algow}
	\end{center}
	\vskip 0in
\end{figure}

where
\begin{equation}
	\begin{array}{l}
		{{\rm B}^{a,b}}\left( {x_i^m,x_i^1,x_i^2,x_i^3} \right) = \\
		{F_{co}}\left[ {f_w^{a,b}\left( {x_i^m} \right),{f_\vartheta }\left( {{f_\omega }\left( {x_i^1} \right)} \right),{f_\vartheta }\left( {{f_\omega }\left( {x_i^2} \right)} \right),{f_\vartheta }\left( {{f_\omega }\left( {x_i^3} \right)} \right)} \right]
	\end{array}
\end{equation}

Then we impose statistical constraints onto the learned embedding by implicitly training the encoder so that the push-forward distribution ${{{\mathcal{U}_{\vartheta,\omega,\mathcal{P}}^*}}}$ matches a prior $\mathcal{V^*}$. To do this, we first sample several samples from the prior $\mathcal{V^*}$. Based on the discrimination network ${D_\phi ^*}$, optimization is applied as follows:
\begin{equation}
	\begin{array}{l}
		\mathop {\min }\limits_{{f_\omega },{f_\vartheta }}\mathop {\max }\limits_{D_\phi ^*} D\left( {\mathcal{V}\left| {{{\mathcal{U}_{\vartheta,\omega,\mathcal{P}}^*}}} \right.} \right) =\\
		\mathop \mathbb{E} \limits_{{x_v} \sim {\mathcal V^*}} \left( {\log D_\phi ^*\left( {{x_v}} \right)} \right) + \mathop \mathbb{E} \limits_{x_i^m \sim P\left( {{X^m}} \right),\hfill\atop
			m \in \left\{ {1,2,3} \right\}\hfill} \left( {1 - D_\phi ^*\left( {{f_\vartheta }\left( {{f_\omega }\left( {x_i^m} \right)} \right)} \right)} \right)
	\end{array}.
\end{equation}

Based on above, the objective function of $Full-View$ is defined as:
\begin{equation}
	\mathop {\max }\limits_{{f_\omega },{f_\vartheta },{D_\phi^*}, V_w^G,V_w^L }{L_{fv}} = \bar I_{global}^{JSD} + \bar I_{local}^{JSD} - \bar D\left( {\mathcal{V}\left| {{{\mathcal{U}_{\vartheta,\omega,\mathcal{P}}^*}}} \right.} \right).
\end{equation}

Lastly, the objective function of local consistency module is defined as:
\begin{equation}
	\mathop {\max }\limits_{{f_\omega },{f_\vartheta },{D_\phi},{D_\phi^*},T_w^G,T_w^L,V_w^G,V_w^L}{L_{lc}} = {\alpha \cdot L_{fv}} + {\beta \cdot L_{iv}}
\end{equation}
where $\alpha$ and $\beta$ are the hyper-parameters for $L_{fv}$ and $L_{iv}$.

\subsection{Versatile view consistency preserving network}
Following the framework of our proposed \textit{local consistency and global alignment network} (LCGAN) in Figure \ref{fig:algoframe}, we incorporate the local consistency and the global alignment objectives. Overall, our complete objective for the proposed LCGAN is defined as:
\begin{equation}
\label{equal16}
\mathop {\max }\limits_{{f_\omega },{f_\vartheta },{D_\phi},{D_\phi^*},T_w^G,T_w^L,V_w^G,V_w^L,\xi_{12},\xi_{13},\xi_{23}}L_{LCGAN}={L_{lc}} - {\gamma \cdot L_{ga}}
\end{equation}
where $\gamma$ is the coefficient that controls the balance between $L_{lc}$ and $L_{ga}$. Furthermore, we conduct experiments to study the influence of $\alpha$, $\beta$, and $\gamma$, respectively. As we can see, maximizing the first term of equation \ref{equal16} can make the multi-view representations consistent in a local manner, and maximizing the second term of equation \ref{equal16} can make the representations aligned globally.

